Goal Space Abstraction in Hierarchical Reinforcement Learning via Set-Based Reachability Analysis

Open-ended learning benefits immensely from the use of symbolic methods for goal representation as they offer ways to structure knowledge for efficient and transferable learning. However, the existing Hierarchical Reinforcement Learning (HRL) approaches relying on symbolic reasoning are often limited as they require a manual goal representation. The challenge in autonomously discovering a symbolic goal representation is that it must preserve critical information, such as the environment dynamics. In this paper, we propose a developmental mechanism for goal discovery via an emergent representation that abstracts (i.e., groups together) sets of environment states that have similar roles in the task. We introduce a Feudal HRL algorithm that concurrently learns both the goal representation and a hierarchical policy. The algorithm uses symbolic reachability analysis for neural networks to approximate the transition relation among sets of states and to refine the goal representation. We evaluate our approach on complex navigation tasks, showing the learned representation is interpretable, transferrable and results in data efficient learning.

==> planning.tex <==
\section{Model-based high-level goal sampling}
\label{sec:planning}
\acronym learns a transition relation between subgoals in the task. The Q-learning approach currently implemented in the high-level agent does not explicitly utilise these relations when selecting subgoals. Instead, such representation lends itself to more informed subgoal sampling strategies such as planning, which can sample long trajectories directly from the subgoal space.% and achieve more efficient learning.
% In this section, we demonstrate that the 

We substitute the Q-Learning algorithm learning the high-level policy in \acronym with a simple planning algorithm inspired by \cite{DBLP:conf/nips/EysenbachSL19} (we call such version \acronym-Planning).
We build a directed graph $H = (V,E)$ where nodes are subgoals $V = \mathcal{G}$ and edges are possible transitions inferred from the memory $\mathcal{D}^{\text{High}}$. By design of the representation and Eq. \eqref{eq:prop}, each transition $(G_i, G_j)$ corresponds to a maximum of $k$ steps in the environment. In addition, the edges $(G_i, G_j)$ are weighted wrt the maximum environment reward obtained when transitioning from $G_i$ to $G_j$ as such $w_{G_i, G_j} = \frac{1}{1+max(r^{ext})}$. When in a state $s \in G_i$, the high-level agent finds the shortest path in $H$, which in our context approximate the highest rewarding trajectory, achievable in the least amount of steps.

We evaluate \acronym-Planning on the 2 Paths Maze configuration (Fig. \ref{fig:maze}). In such configuration there are two ways to solve the maze: from the starting position the agent can either take the upper path, which is harder to train a low-level policy for, or take the narrow, harder to discover, shorter path at the bottom.
From Fig. \ref{fig:config3} we see that using the planning component achieves a superior performance for such environment. The high-level agent samples more goals passing through the bottom shortcut achieving %a high data efficiency,
faster low-level training.% and subgoal representation.
\acronym without planning, instead, favors the more commonly encountered upper path and thus achieves sub-optimal performance.
The obtained subgoal representation by the planning approach is shown in Fig. \ref{fig:config3_repr}, while the graph in Fig. \ref{fig:graph} shows the connected transitions in the learned partitions. The shortest path in this graph corresponds to 6,0,4,8,16. We note that, the extracted graph only features subgoals and transitions depending on the agent's exploration and reachability analysis, which explains why not all conceptually possible transitions are in the graph.

\begin{figure*}[tbh]
  \begin{center}
    \subfloat[Subgoals decomposition \label{plan_repr}]{%
      \includegraphics[width=0.32\textwidth]{figs/repr_planning.png}
    }
    %
    \hfill
    \subfloat[Evaluation\label{fig:config3}]{
    \includegraphics[width=0.62\textwidth]{figs/Figure_8.png}
    }\\    
    %
    \subfloat[Extracted Graph \label{fig:graph}]{%
      \includegraphics[width=0.7\textwidth]{texfigs/graphs_2_paths_maze.pdf}
    }
  \end{center}
  \vspace{-0.4cm}
  \caption{Representations and evaluation of \acronym-Planning on the 2 Paths Maze.}
  \label{fig:config3_repr}
\end{figure*}

